Learning to Ignore: Fair and Task Independent Representations

Training fair machine learning models, aiming for their interpretability and solving the problem of domain shift has gained a lot of interest in the last years. There is a vast amount of work addressing these topics, mostly in separation. In this work we show that they can be seen as a common framework of learning invariant representations. The representations should allow to predict the target while at the same time being invariant to sensitive attributes which split the dataset into subgroups. Our approach is based on the simple observation that it is impossible for any learning algorithm to differentiate samples if they have the same feature representation. This is formulated as an additional loss (regularizer) enforcing a common feature representation across subgroups. We apply it to learn fair models and interpret the influence of the sensitive attribute. Furthermore it can be used for domain adaptation, transferring knowledge and learning effectively from very few examples. In all applications it is essential not only to learn to predict the target, but also to learn what to ignore.

==> relatedWork.tex <==
\todo{LINDA: ich hab da recht gestrichen -- nicht sicher ob das alles noch so sinn macht -- bitte checken und ev. finden wir noch 1-2 mehr refs dazu...}
\paragraph{Fairness.}
%Fairness in machine learning nowadays has become a societal focus and a lot of work goes into different approaches to make neural networks "fair" in certain aspects. The goal in general is to learn data representations where the semantics of the characteristics introducing a bias are removed. For accomplishing this task, there are mainly two different approaches.
In order to make machine learning models "fair" work aim for modifying the feature representations of the data~\cite{Zemel2013}, the class label annotations~\cite{ThanhLuong2011} or the data itself~\cite{Quadrianto}.
%For example Zemel et al.~ \cite{Zemel2013} use a probabilistic mapping of the data points to a new representation space which is independent of the sensitive attribute. %Adversarial Learning is another way of removing sensitive information from a latent representation learned by a neural network. This is done for example with an 
Learning this latent representation includes an additional cross entropy classification loss~\cite{Beutel}, a decomposition loss~\cite{Quadrianto}, an additional hidden layer for adversarial optimization~\cite{Adel}, using Variational Autoencoders~\cite{Louizos}, or by learning the representation as an adversarial minimax game~\cite{Xie}. The goal is not only to improve fairness but also the possibility of interpreting how fairness is enforced.

\paragraph{Interpretability/ Causality.}
Understanding and interpreting (causal) relationships in neural networks is important for getting a better and deeper understanding of the learned representation. Methods aiming to reach causal inference includes special network architectures~\cite{Chattopadhyay2019}, Variational Autoencoders~\cite{Louizos2017}, or combination of different machine learning algorithms~\cite{Hartford2016}. If causal aspects are taken into account, predictions can be improved~\cite{Buhlmann2018}. This is also the reason why this area is getting more and more attention.
%take a more general approach showing how to combine different machine learning algorithms by introducing a causal framework.

\paragraph{Domain Adaptation and Generalization.}
%The problem with a common neural network trained on only one data set is rather poor performance on new data from another domain or distribution. In general, there exist two main techniques to counteract this issue aiming at slightly different targets. The first and widely researched field is 
Domain adaptation uses additionally (unlabeled) samples from the target domain. Domain generalization learns a model from multiple sources that then can be applied to other (target) domains. Approaches make use of re-weighting the source samples to better match the target domain~\cite{Huang,Pinheiro2018}, learning shared weights~\cite{Yang}, learning a common subspace~\cite{Ganin2017}, modifying the network architecture~\cite{Mancini2018, Motiian2017}, or using Generative Adversarial Networks~\cite{Louizos,Ghifary}

%Instance-based methods use a re-weighting of the source samples according to the similarity with a target domain \cite{Huang,Pinheiro2018}. Feature-based methods learn a common subspace for source and target data to obtain domain-invariant representations. This common subspace can for example be achieved by introducing new layers to the neural nets \cite{Ganin2017} or even a new Convolutional Neural Network (CNN) architecture which then can be included as a side branch or as novel layers on top of an existing network \cite{Mancini2018}. Parameter-based approach which uses a set of shared weights between source and target model \cite{Yang}. Deep architectures such as generative adversarial networks or deep autoencoders \cite{Louizos,Ghifary} have shown success in domain adaptation as well as in generalization. \cite{Motiian2017} using a Siamese architecture for both domain adaptation as well as generalization.
